Deconstructing Instruction-Following: A New Benchmark for Granular Evaluation of Large Language Model Instruction Compliance Abilities

Reliably ensuring Large Language Models (LLMs) follow complex instructions is a critical challenge, as existing benchmarks often fail to reflect real-world use or isolate compliance from task success. We introduce MOSAIC (MOdular Synthetic Assessment of Instruction Compliance), a modular framework that uses a dynamically generated dataset with up to 20 application-oriented generation constraints to enable a granular and independent analysis of this capability. Our evaluation of five LLMs from different families based on this new benchmark demonstrates that compliance is not a monolithic capability but varies significantly with constraint type, quantity, and position. The analysis reveals model-specific weaknesses, uncovers synergistic and conflicting interactions between instructions, and identifies distinct positional biases such as primacy and recency effects. These granular insights are critical for diagnosing model failures and developing more reliable LLMs for systems that demand strict adherence to complex instructions.

==> sections/improvements.tex <==
\subsection{Constraint Rewriting Workflow}

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{images/Mitigation strategy workflow.png}
\caption{Proposed workflow for prompt refinement to increase instruction following compliance in a constrained text generation task.}
\label{fig:workflow}
\end{figure}
To enhance instruction-following compliance of a model, we propose a novel, multi-agent prompt rewriting system that iteratively refines a modular list of constraints. This system operationalizes three core strategies within an in-context learning framework. First, we strictly decouple the primary text generation task from the list of constraints, allowing the system to focus exclusively on rewriting the instructional components. Second, we use the evaluation metrics defined in Section 3.2 as a direct feedback signal to guide the refinement process. Third, we employ a planner-executor agent architecture to make targeted, intelligent edits to the constraints, aiming to improve the model's compliance.

The workflow, illustrated in Figure~\ref{fig:workflow}, is orchestrated as a stateful graph using LangGraph \footnote{\url{https://www.langchain.com/langgraph}} and consists of four primary stages: (i) Content Generation, (ii) Evaluation, (iii) Action Planning, and (iv) Constraint Editing. This cycle repeats until one of two termination conditions is met: either a maximum number of iterations, $N_{max}$, is reached, or the global compliance score fails to improve for a predefined number of steps, a threshold we term patience $P_{max}$.
The workflow is managed by a series of specialized agents:
\begin{itemize}[nosep]
    \item \textbf{Generator Agent:} Generates text by following the prompt, which contains the primary task description and the \textit{current} version of the constraints.

    \item \textbf{Evaluator Agent:} Leverages the $SCC_c$ and $PA_r$ metrics to assess the Generator agent's output. It calculates both a global compliance score and individual scores for each of the original constraints, providing a quantitative measure of performance.

    \item \textbf{Translator Agent:} Converts the numerical scores from the Evaluator agent into a textual summary. This summary describes how the compliance score for each constraint and the global score have changed relative to the previous iteration (e.g., ``increased'', ``decreased'', or ``unchanged''), creating a qualitative feedback report.

    \item \textbf{Planner Agent:} Functions as the strategic core of the system. It receives the entire history of previous edits, the current set of constraints, and the textual feedback from the Translator agent. Based on this information, it decides which constraint to edit and what action to take, outputting its decision as a detailed instruction. The actions available to this agent are: (i) ``rephrase'' i.e., change the wording of one constraint; (ii) ``split'' i.e., divide a long constraint into multiple short ones; (iii) ``merge'' i.e., combine multiple short constraints into a long one.
    \item \textbf{Constraint Editing Agent:} Receives the instruction from the Planner agent and performs the actual modification, rewriting the list of constraints. The resulting new set of constraints is then passed to the Generator agent in the next iteration.
\end{itemize}



%
%
%
%
%
%\subsection{Instruction Following Compliance Improvement Strategies}
%\begin{figure*}[h!]
%\includegraphics[width=\linewidth]{images/Mitigation strategy workflow.png}
%\caption{Proposed workflow for prompt refinement to increase instruction following in the constrained text generation task.}
%\label{fig:workflow}
%\end{figure*}
%We propose a novel four-stage prompt rewriting system targeting a modular list of constraints. The system incorporates three major improvement strategies into the framework of in-context reinforcement learning. First, we decouple the task from the list of constraints to help LLM focus on constraint \textcolor{red}{and task description} rewriting. Second, we adopt our evaluation functions to guide the selection of refinement actions. Finally, we introduce a finite set of refinement actions to regulate LLM's behavior and increase compliance.

%Consider a task $T$ and a list of initial constraints, we define their formulations at each refinement step $i$ as:
%\begin{equation}
%\mathbf{C}^{(i)} = \left[C_1^{(i)}, C_2^{(i)}, ..., C_K^{(i)}\right].
%\end{equation}
%where $C_k^{(i)}$ is the $k$-th constraint for $k = 1, 2, ..., K$ in its $i-th$ formulation for $i = 0, 1, .. N$ computed by the proposed workflow. 

%\textbf{Notations}. Consider a task $T$ and a list of initial constraints:
%\begin{equation}
%\mathbf{C}^{(0)} = \left[C_1^{(0)}, C_2^{(0)}, ..., C_K^{(0)}\right].
%\end{equation}
%where $C_k^{(0)}$ is the $k$-th initial constraint for $k = 1, 2, ..., K$ in its original formulation -- denoted by the $^{(0)}$. We now define the notations for the $i$-th iteration of refinement in the following:
%\begin{itemize}
%\item The list of refined constraints,
%\begin{equation}
%\tilde{\mathbf{C}}^{(i)} = \left[\tilde{C}_1^{(i)}, \tilde{C}_2^{(i)}, ..., \tilde{C}_K^{(i)}\right].
%\end{equation}
%
%\item The prompt generated by a template $f$,
%\begin{equation}
%P^{(i)} = f\left(T, \tilde{\mathbf{C}}^{(i)}\right).
%\end{equation}
%
%\item The response corresponding to $P^{(i)}$,
%\begin{equation}
%R^{(i)} = LLM\left(P^{(i)}\right).
%\end{equation}
%
%\item The local compliance score generated by the evaluation function $g_k$ for $C_k^{(0)}$, 
%\begin{equation}
%S_k^{(i)} = g_k\left(R^{(i)}\right).
%\end{equation}
%
%\item The global compliance score generated by aggregating $K$ local scores through a function $h$,
%\begin{equation}
%S^{(i)} = h\left(S_k^{(i)}\right).
%\end{equation}
%
%\item The refinement action $a_k^{(i)}$ selected from a finite set $\mathbf{A}$ for $\tilde{C}_k^{(i)}$,
%\begin{equation}
%a_k^{(i)} \in \mathbf{A} = \{a_1, a_2, ..., a_n\},
%\end{equation}
%such that
%\begin{equation}
%\tilde{\mathbf{C}}^{(i+1)} = \left[\tilde{C}_1^{(i)}, ..., a_k^{(i)}\left(\tilde{C}_k^{(i)}\right), ..., \tilde{C}_K^{(i)}\right].
%\end{equation}
%
%\end{itemize}

%
%The workflow we propose, as illustrated in Figure \ref{fig:workflow} consists of the following stages: (i) Evaluation, (ii) Action Planning, (iii) Constraint Editing, (iv) Content Generation. This process is repeated $N$ times or until the Action Planning agent decides to conclude it. The workflow relies on the following agents:
%
%\begin{itemize}[nosep]
%
%\item \textbf{Evaluation agent.} Leverages the metrics we described in the previous sections to evaluate the instruction compliance rate associated with a response and a given list of constraints it has to comply with. 
%
%\item \textbf{Action Planning agent. } Receives the compliance metrics provided by the Evaluation agent and decides (i) which constraint to edit and (ii) what edit action to take. We allow this agent to choose between rephrasing one constraint or to change its rank in the prompt. This agent may also decide not to further edit the prompt and to exit the refinement loop.
%
%\item \textbf{Rephrase agent.} Rephrases a constraint based on its original formulation and the prompt containing it.
%
%\item \textbf{Reorder agent.} Decides the new rank of a constraint in the list of constraints associated with a prompt. This decision is based on the prompt, the list of other constraints, the performance metrics associated with all of the constraints in the prompt based on a training set.
%
%\item \textbf{Content Generation agent.} Generates content complying with a prompt containing a list of constraints with different formulations.
%\end{itemize}

%
%\textbf{Workflow}. The system, as illustrated in Figure \ref{fig:workflow} consists of two stages: the evaluation stage and the refinement stage. The stages are driven by two respective LLM agents: evaluator and refiner.
%
%The evaluator leverages rule-based functions to evaluate all the formatting constraints and most of the lexcial constraints in Table \ref{tab:constraints}, and LLM-based functions (LLM-as-a-judge) to evaluate the other constraints. The evaluator is a memoryful agent in that it memorizes the compliance scores for the last iteration in order to quantify the deltas. Given the prompt $P^{(i)}$, the response $R^{(i)}$ and the refinement action $a_k^{(i)}$ for the $i$-th iteration, the evaluator first calculates the local compliance scores, $S_1^{(i)}, S_2^{(i)}, ..., S_k^{(i)}$ and the global compliance score $S^{(i)}$. For simplicity, we choose the mean function to be the aggregation function $h$ for calculating the global compliance score. Next, the evaluator computes the deltas between the scores for the $i$-th and $(i-1)$-th iterations as the following,
%\begin{align}
%\Delta_k^{(i)} & = S_k^{(i)} - S_k^{(i-1)},\\
%\Delta^{(i)} & = S^{(i)} - S^{(i-1)}.
%\end{align}
%Then the evaluator translates the results into a compliance report as shown in the example below.\\
%\noindent \texttt{\small
%For iteration <$i$>, the refinement action <$a_k^{(i)}$> is applied to the constraint <$\tilde{C}_k^{(i)}$>, which achieves the following scores:\\
%<$S_1^{(i)}$> in compliance with the constraint <$C_1^{(0)}$>, <increasing/decreasing> from the last iteration by <$\Delta_1^{(i)}$>.\\
%...\\
%<$S_K^{(i)}$> in compliance with the constraint <$C_K^{(0)}$>, <increasing/decreasing> from the last iteration by <$\Delta_K^{(i)}$>.\\
%Overall, the compliance score is <$S^{(i)}$>, <increasing/decreasing> from last iteration by <$\Delta^{(i)}$>.}\\
%Finally, if the global compliance score is higher than a pre-specified threshold $\tau$ or the maximum number of iterations $M$ is reached, the evaluator returns $P^{(M)}$ as the final output. Otherwise, the evaluator passes both the report and the constraint that has the lowest local compliance score to the refiner.
%
%Similar to the evaluator, the refiner is also memoryful in that it maintains a history of refinement for every iteration to provide a richer context for action selection and encourage better decision making. The history of refinement is initialized by an empty list. Given the task $T$, the compliance report and the constraint that has the lowest local compliance score from the evaluator, the refiner appends the compliance report to the end of the history and applies the best action to the constraint with the hope of maximizing both the local and global compliance scores. Finally, the refiner starts the next iteration by passing the list of refined constraints $\tilde{\mathbf{C}}^{(i+1)}$ back to the evaluator.
